NeuManifold: Neural Watertight Manifold Reconstruction with Efficient and High-Quality Rendering Support

We present a method for generating high-quality watertight manifold meshes from multi-view input images. Existing volumetric rendering methods are robust in optimization but tend to generate noisy meshes with poor topology. Differentiable rasterization-based methods can generate high-quality meshes but are sensitive to initialization. Our method combines the benefits of both worlds; we take the geometry initialization obtained from neural volumetric fields, and further optimize the geometry as well as a compact neural texture representation with differentiable rasterizers. Through extensive experiments, we demonstrate that our method can generate accurate mesh reconstructions with faithful appearance that are comparable to previous volume rendering methods while being an order of magnitude faster in rendering. We also show that our generated mesh and neural texture reconstruction is compatible with existing graphics pipelines and enables downstream 3D applications such as simulation. Project page: https://sarahweiii.github.io/neumanifold/

==> tables/quality_speed.tex <==
% \setlength{\tabcolsep}{4pt}
\begin{table}
\small
\caption{Trade-off between rendering speed and quality with different appearance network capacity. 8$\times$ MS: 8$\times$ sample per-pixel MSAA, 16$\times$ SS: 16$\times$ sample per-pixel SSAA. (SH: Spherical Harmonics)
\label{tab:trade-off}
\vspace{-1em}
\begin{tabular}{l|c|c|ccc|c}
\toprule
Model & Params & AA & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & FPS \\
\midrule
\multirow{2}{*}{Ours-F} & \#feat=48 & 8$\times$ MS & 29.73 & 0.943 & 0.068 & 312 \\
 &  SH & 16$\times$ SS & 30.44 & 0.949 & 0.063 & 82 \\
\midrule
\multirow{2}{*}{Ours} & \#feat=48 & 8$\times$ MS & 30.34 & 0.949 & 0.062 & 93 \\
 & MLP=3$\times$64 & 16$\times$ SS & 31.16 & 0.954 & 0.057 & 26 \\
 \bottomrule
\end{tabular}

\vspace{-1em}
\end{table} 
